Product Configuration in Answer Set Programming

This is a preliminary work on configuration knowledge representation which serves as a foundation for building interactive configuration systems in Answer Set programming (ASP). The major concepts of the product configuration problem are identified and discussed with a bike configuration example. A fact format is developed for expressing product knowledge that is domain-specific and can be mapped from other systems. Finally, a domain-independent ASP encoding is provided that represents the concepts in the configuration problem.

==> abstract.tex <==
\begin{abstract}
    \textbf{Abstract.} This is a preliminary work on configuration knowledge representation which serves as a foundation for building interactive configuration systems in Answer Set Programming (ASP).
    The major concepts of the product configuration problem are identified and discussed with a bike configuration example.
    A fact format is developed for expressing product knowledge that is domain-specific and can be mapped from other systems. 
    Finally, a domain-independent ASP encoding is provided that represents the concepts in the configuration problem.
\end{abstract}


==> eptcsdata.tex <==
\providecommand{\firstpage}{296}
\providecommand{\publicationstatus}{A. Formisano, Y.A Liu, et al. (Eds.): International Conference on\\ Logic Programming (Technical Communications) 2021 (ICLP 2021)\\
EPTCS 345, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.345.46}{10.4204/EPTCS.345.46}}
\pdfoutput=1

